L-Dunford-Pettis property in Banach spaces

In this paper, we introduce and study the concept of L-Dunford-Pettis sets and L-Dunford-Pettis property in Banach spaces. Next, we give a characterization of the L-Dunford-Pettis property with respect to some well-known geometric properties of Banach spaces. Finally, some complementability of operators on Banach spaces with the L-Dunford-Pettis property are also investigated

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{4}

